Wolf: Dense Video Captioning with a World Summarization Framework

We propose Wolf, a WOrLd summarization Framework for accurate video captioning. Wolf is an automated captioning framework that adopts a mixture-of-experts approach, leveraging complementary strengths of Vision Language Models (VLMs). By utilizing both image and video models, our framework captures different levels of information and summarizes them efficiently. Our approach can be applied to enhance video understanding, auto-labeling, and captioning. To evaluate caption quality, we introduce CapScore, an LLM-based metric to assess the similarity and quality of generated captions compared to the ground truth captions. We further build four human-annotated datasets in three domains: autonomous driving, general scenes, and robotics, to facilitate comprehensive comparisons. We show that Wolf achieves superior captioning performance compared to state-of-the-art approaches from the research community (VILA1.5, CogAgent) and commercial solutions (Gemini-Pro-1.5, GPT-4V). For instance, in comparison with GPT-4V, Wolf improves CapScore both quality-wise by 55.6% and similarity-wise by 77.4% on challenging driving videos. Finally, we establish a benchmark for video captioning and introduce a leaderboard, aiming to accelerate advancements in video understanding, captioning, and data alignment. Webpage: https://wolfv0.github.io/.

==> imgs/finetune/figure.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.35\textwidth]{imgs/finetune/finetune.pdf}

    \caption{Comparison on 500 highly interactive Nuscenes videos VILA-1.5 and fine-tuned VILA-1.5 with \method{} captions. }
    \label{fig:finetune}

\end{figure}


==> tables/capscore_com.tex <==
\begin{table}[]

\begin{center}

\scalebox{0.8}{

\begin{tabular}{l|c|c|c|c}
\toprule
{Model}&  {CLIP-Score} $\uparrow$& {CapScore$_S$}$\uparrow$&{CapScore$_Q$}$\uparrow$&N-avg$\uparrow$\\ 
\midrule
MiniGPT-4  &\underline{0.601} &0.330&0.359&0.19\\
InstructBLIP & 0.599&0.360&0.355&0.18 \\
LLaVA-1.5 & \underline{0.601}&\underline{0.385}&\textbf{0.450}&\underline{0.67} \\
mPLUG-Owl2 & 0.597&\textbf{0.397}&0.400&0.49 \\
Qwen2-VL & \textbf{0.618}&0.373&\underline{0.432}&\textbf{0.82} \\
\bottomrule
\end{tabular} 
}

\end{center}

\caption{Comparison on CapScore and CLIP-Score for text-image alignment. CapScore$_S$ represents CapScore Similarity; {CapScore$_Q$} represents CapScore Quality (such as reduced hallucination); N-avg represents noun/verb average. We observe that CapScore aligns with trends observed in other metrics but highlights a larger performance gap between models, suggesting it serves as a more effective evaluation metric. Note: All scores are scaled to the range [0, 1].}
\label{tab:capscorecom}
\vspace{-0.15in}
\end{table}


